Simulating rare kaon decays $K^{+}\to\pi^{+}\ell^{+}\ell^{-}$ using domain wall lattice QCD with physical light quark masses

We report the first calculation using physical light-quark masses of the electromagnetic form factor $V(z)$ describing the long-distance contributions to the $K^+\to\pi^+\ell^+\ell^-$ decay amplitude. The calculation is performed on a 2+1 flavor domain wall fermion ensemble with inverse lattice spacing $a^{-1}=1.730(4)$GeV. We implement a Glashow-Iliopoulos-Maiani cancellation by extrapolating to the physical charm-quark mass from three below-charm masses. We obtain $V(z=0.013(2))=-0.87(4.44)$, achieving a bound for the value. The large statistical error arises from stochastically estimated quark loops.

==> Rare Kaon Decays/suppMat.tex <==



%\keywords{Suggested keywords}%Use showkeys class option if keyword
                              %display desired




\begin{figure*}
    \begin{minipage}{1.5in}
\setlength{\unitlength}{.05in}
        \begin{picture}(55,40)(0,0)
        \multiput(-33,35)(10,0){1}{\circle*{2}}
        \put(-30,39){\makebox(0,0)[r]{\small{(0,0)}}}
        \multiput(-23,35)(10,0){1}{\circle{2}}
        \put(-20,39){\makebox(0,0)[r]{\small{(0,1)}}}
        \multiput(-13,35)(10,0){1}{\circle*{2}}
        \put(-10,39){\makebox(0,0)[r]{\small{(0,2)}}}
        \multiput(-3,35)(10,0){1}{\circle{2}}
        \put(0,39){\makebox(0,0)[r]{\small{(0,3)}}}
        \multiput(-33,25)(10,0){1}{\circle{2}}
        \put(-30,29){\makebox(0,0)[r]{\small{(1,0)}}}
        \multiput(-23,25)(10,0){1}{\circle{2}}
        \put(-20,29){\makebox(0,0)[r]{\small{(1,1)}}}
        \multiput(-13,25)(10,0){1}{\circle{2}}
        \put(-10,29){\makebox(0,0)[r]{\small{(1,2)}}}
        \multiput(-3,25)(10,0){1}{\circle{2}}
        \put(0,29){\makebox(0,0)[r]{\small{(1,3)}}}
        \multiput(-33,15)(10,0){1}{\circle*{2}}
        \put(-30,19){\makebox(0,0)[r]{\small{(2,0)}}}
        \multiput(-23,15)(10,0){1}{\circle{2}}
        \put(-20,19){\makebox(0,0)[r]{\small{(2,1)}}}
        \multiput(-13,15)(10,0){1}{\circle*{2}}
        \put(-10,19){\makebox(0,0)[r]{\small{(2,2)}}}
        \multiput(-3,15)(10,0){1}{\circle{2}}
        \put(0,19){\makebox(0,0)[r]{\small{(2,3)}}}
        \multiput(-33,5)(10,0){1}{\circle{2}}
        \put(-30,9){\makebox(0,0)[r]{\small{(3,0)}}}
        \multiput(-23,5)(10,0){1}{\circle{2}}
        \put(-20,9){\makebox(0,0)[r]{\small{(3,1)}}}
        \multiput(-13,5)(10,0){1}{\circle{2}}
        \put(-10,9){\makebox(0,0)[r]{\small{(3,2)}}}
        \multiput(-3,5)(10,0){1}{\circle{2}}
        \put(0,9){\makebox(0,0)[r]{\small{(3,3)}}}

        \put(10,3){\line(0,1){39}} % vert line

        \put(5.5,23){\vector(1,0){10}}
        \put(13,29){\makebox(0,0)[r]{shift}}
        \put(14,26){\makebox(0,0)[r]{y-dim}}


        \multiput(23,35)(10,0){1}{\circle{2}}
        \put(26,39){\makebox(0,0)[r]{\small{(0,0)}}}
        \multiput(33,35)(10,0){1}{\circle{2}}
        \put(36,39){\makebox(0,0)[r]{\small{(0,1)}}}
        \multiput(43,35)(10,0){1}{\circle{2}}
        \put(46,39){\makebox(0,0)[r]{\small{(0,2)}}}
        \multiput(53,35)(10,0){1}{\circle{2}}
        \put(56,39){\makebox(0,0)[r]{\small{(0,3)}}}
        \multiput(23,25)(10,0){1}{\circle*{2}}
        \put(26,29){\makebox(0,0)[r]{\small{(1,0)}}}
        \multiput(33,25)(10,0){1}{\circle{2}}
        \put(36,29){\makebox(0,0)[r]{\small{(1,1)}}}
        \multiput(43,25)(10,0){1}{\circle*{2}}
        \put(46,29){\makebox(0,0)[r]{\small{(1,2)}}}
        \multiput(53,25)(10,0){1}{\circle{2}}
        \put(56,29){\makebox(0,0)[r]{\small{(1,3)}}}
        \multiput(23,15)(10,0){1}{\circle{2}}
        \put(26,19){\makebox(0,0)[r]{\small{(2,0)}}}
        \multiput(33,15)(10,0){1}{\circle{2}}
        \put(36,19){\makebox(0,0)[r]{\small{(2,1)}}}
        \multiput(43,15)(10,0){1}{\circle{2}}
        \put(46,19){\makebox(0,0)[r]{\small{(2,2)}}}
        \multiput(53,15)(10,0){1}{\circle{2}}
        \put(56,19){\makebox(0,0)[r]{\small{(2,3)}}}
        \multiput(23,5)(10,0){1}{\circle*{2}}
        \put(26,9){\makebox(0,0)[r]{\small{(3,0)}}}
        \multiput(33,5)(10,0){1}{\circle{2}}
        \put(36,9){\makebox(0,0)[r]{\small{(3,1)}}}
        \multiput(43,5)(10,0){1}{\circle*{2}}
        \put(46,9){\makebox(0,0)[r]{\small{(3,2)}}}
        \multiput(53,5)(10,0){1}{\circle{2}}
        \put(56,9){\makebox(0,0)[r]{\small{(3,3)}}}
        \end{picture}
\end{minipage}
        \caption{An example of sparse noises for $d=2$, $n=2$. The filled circles represent a site with $Z_{2}$ noise, the empty circles represent a site that has been set to zero. Two further shifts are needed to cover the full volume, giving $2^2=4$ sparse sources.}
    \label{fig:sparse_noise_example}
\end{figure*}

\section{\label{sec:sparse_sources}Sparse Sources}
The spacetime distribution of a source may be treated stochastically, in order to decrease the effects of local fluctuations from the gauge fields. This is important for constructing lattice propagators of the form $S\left({x,x}\right)$, which are needed to calculate a disconnected diagram or a single-propagator trace contribution to a correlation function, needed for the Eye and Saucer diagrams (Fig.~\ref{fig:H_W_contractions}) contributing to the rare kaon decay amplitude. To create the propagators we depend on $N$ stochastic sources $\kappa_{i}$ that fulfill the properties
\begin{equation}
\label{eq:stoch_source_props}
\begin{split}
    \lim_{N\to\infty}&\frac{1}{N}\sum_{i=1}^{N} \kappa_{i}\left({x}\right) = 0, \\
    \lim_{N\to\infty}&\frac{1}{N}\sum_{i=1}^{N} \kappa_{i}\left({x}\right)\kappa_{i}^{\dagger}\left({y}\right) = \delta_{xy}.
\end{split}
\end{equation}
One appropriate choice is the $Z_{2}$ source \cite{Z2noise}, where each element is randomly chosen from
\begin{equation}
\label{eq:z2_source_defn}
    Z_{2}\otimes Z_{2} = \left\{\frac{1}{\sqrt{2}}\left({\pm1\pm i}\right)\right\}.
\end{equation}

It is expected that the statistical error introduced from using stochastic sources scales as ${1}/{\sqrt{N}}$. Each stochastic source here covers the full volume but we can also create ``sparse sources'', similar to those described in \cite{PhysRevLett.116.232002}, to improve the ${1}/{\sqrt{N}}$ scaling of the statistical error. In $d$-dimensional spacetime we create $N=n^{d}$ sparse sources where
\begin{equation}
\label{eq:sparse_sources_defn}
    \kappa_{\textrm{sparse}}(x) = 
       \begin{cases}
            \kappa_{Z_{2}}(x):  x_{\mu} ~\mathrm{ mod }~ n = 0, \quad \mu=0,1,2,3 \\
            0: \mathrm{otherwise} \\
        \end{cases}
\end{equation}
for the first source and we shift in each dimension to ensure that the N sources cover the entire volume with no overlap when combined, see Fig.~\ref{fig:sparse_noise_example} for a $d=2$, $n=2$ example. When investigating rare kaon decays we use $N=2^{4}=16$ sparse sources for each hit of a propagator, $S\left({x,x}\right)$, that we compute.\\
A cost-benefit analysis was performed using the quantity $\frac{\Delta X}{\Delta{\textrm{Sparse}}}\sqrt{\frac{N_{X}}{N_{{\textrm{Sparse}}}}}$, where ${\Delta X}$ is the statistical error of the result from method $X$ and the root of the number of inversions $N_{X}$ tracks the computational cost of using method $X$. Fig.~\ref{fig:sparseCost} shows the results of this cost-benefit analysis for the 3-point Saucer diagram with zero momentum. The loop in the diagram was computed using sparse sources, full volume sources and time-diluted all-to-all vectors  \cite{A2APractical} with 2000 low modes, with the other propagators being computed with Coulomb-gauge fixed wall sources. This was performed on RBC/UKQCD's $48^3\times96$ M\"obius domain wall fermion gauge ensembles \cite{PhysRevD.93.074505}. It can clearly be seen that the sparse-noise approach is the most successful.
\begin{figure*}
    \begin{centering}
        \includegraphics[width=0.75\textwidth]{./figures/costSources}
    \par\end{centering}
\protect\caption{\label{fig:sparseCost}The statistical error relative to that of the ``Sparse: 16'' noise, weighted by the cost of inversions, of the zero-momentum Saucer diagram contribution to the 3-point weak Hamiltonian correlation function, computed using different noise strategies for the single quark propagator loop.}
\end{figure*}


\begin{figure*}
    \begin{centering}
    	\begin{tabular}{cccc}
    		\includegraphics[scale=0.6]{figures/feyn_W.pdf} & \includegraphics[scale=0.6]{figures/feyn_C.pdf} & \includegraphics[scale=0.6]{figures/feyn_S.pdf} & \includegraphics[scale=0.6]{figures/feyn_E.pdf}\tabularnewline
    		$W$ & $C$ & $S$ & $E$\tabularnewline
    		(Wing) & (Connected) & (Saucer) & (Eye)\tabularnewline
    	\end{tabular}
	\par\end{centering}
\protect\caption{\label{fig:H_W_contractions}The four classes of diagrams obtained after performing the Wick contractions of the charged pion and kaon interpolating operators with the $H_{W}$ operator. $\ell$ denotes a light ($u$ or $d$) quark propagator. The two black circles represent the currents in the four-quark operators $Q_{1,2}^{q}$ defined in the main paper. %(\ref{eq:Q1_Q2_definition}).  
The C and E diagrams contain an insertion of $Q_{1}^{q}$ and the W and S diagrams contain an insertion of $Q_{2}^{q}$.}
\end{figure*}
\begin{figure}
	\begin{centering}
		\begin{tabular}{cc}
			\includegraphics[scale=0.6]{figures/feyn_C_Kl.pdf} & \includegraphics[scale=0.6]{figures/feyn_C_Ksb.pdf} \tabularnewline
			\includegraphics[scale=0.6]{figures/feyn_C_pil.pdf} & \includegraphics[scale=0.6]{figures/feyn_C_pilb.pdf} \tabularnewline
		\end{tabular}
			\includegraphics[scale=0.6]{figures/feyn_C_dis.pdf}
		\par\end{centering}
	\caption{\label{fig:Connected_J_contractions}The five possible current insertions for the $C$ class of diagrams contributing to the 4pt rare kaon decay correlator. %(\ref{eq:4pt_corr). 
	The diagrammatic conventions are the same as in Fig.~\ref{fig:H_W_contractions}}
\end{figure}


\section{\label{relevant_corrs}Further relevant correlators}
Before giving details on the fit parameters that were used we outline the definitions of several relevant Euclidean correlation functions.
\subsection{2-point correlators} % (fold)
\label{sub:2point_functions}
Given an interpolation operator $\phi_P(t,\mathbf{p})$ for a pseudoscalar meson, $P$, with spacial momentum $\mathbf{p}$ at time $t$, for $t\gg 0$ the 2-point function
\begin{equation}
    \Gamma^{(2)}_P(t,\mathbf{p})=\langle{\phi_P(t,\mathbf{p})\phi^{\dagger}_P(0,\mathbf{p})}\rangle
\end{equation}
has the following behavior:
\begin{equation}
    \Gamma^{(2)}_P(t,\mathbf{p})=L^{3}\frac{|Z_P(\mathbf{p})|^2}{2E_P(\mathbf{p})}
    [e^{-E_P(\mathbf{p})t} + e^{-E_P(\mathbf{p})(n_t-t)}],
\end{equation}
where $Z_P(\mathbf{p})=\bra{0}\phi_P(0,\mathbf{0})\ket{P(\mathbf{p})}$ and $E_P(\mathbf{p})$ the meson energy $\sqrt{M_P^2+\mathbf{p}^2}$.

We calculated the pion and kaon 2pt functions using Coulomb-gauge fixed wall sources and both Coulomb-gauge fixed wall sinks and point sinks. Although we only require the wall-wall matrix elements in order to extract the decay amplitude the point-wall 2pt functions have a cleaner signal. Thus both the wall-wall and point-wall correlators can be used in a combined fit to obtain $E_P(\mathbf{p})$ with greater accuracy. All pseudoscalar/sink combinations are calculated for $\mathbf{p}=\frac{2\pi}{L}\left(0,0,0\right)$ and $\mathbf{p}=\frac{2\pi}{L}\left(1,0,0\right)$.
% subsection 2point_functions (end)
\subsection{3-point weak Hamiltonian correlator} % (fold)
\label{sub:3_point_h_w}
The weak Hamiltonian 3pt function
\begin{equation}
    \label{eq:3ptHW}
    \Gamma^{(3)}_H(t_H,\mathbf{p})=\int d^3\mathbf{x}\,\langle{\phi_{\pi}(t_{\pi},\mathbf{p})H_W(t_H,\mathbf{x})\phi^{\dagger}_K(0,\mathbf{p})}\rangle
\end{equation}
has the following behavior for $0\ll t_H\ll t_{\pi}$:
\begin{equation}
\begin{split}
    \Gamma^{(3)}_H(t_H,\mathbf{p})=&\,L^3\frac{Z_{\pi}(\mathbf{p})Z_K(\mathbf{p})^{\dagger}\mathcal{M}_H(\mathbf{p})}{4E_{\pi}(\mathbf{p})E_K(\mathbf{p})} \\
                                    & \times e^{-E_{\pi}(\mathbf{p})t_{\pi}}
                                    e^{-[E_K(\mathbf{p})-E_{\pi}(\mathbf{p})]t_H}\,
    \label{eq:GHasymp}
\end{split}
\end{equation} 
with $\mathcal{M}_H(\mathbf{p})=\bra{\pi(\mathbf{p})}H_W(0)\ket{K(\mathbf{p})}$. This correlator is calculated for both $\mathbf{p}=\frac{2\pi}{L}\left(0,0,0\right)$ and $\mathbf{p}=\frac{2\pi}{L}\left(1,0,0\right)$.
% subsection 3_pont_h_w (end)
\subsection{3-point electromagnetic current correlator} % (fold)
\label{sub:3_point_electromagnetic_current}
The electromagnetic current 3pt function for a pseudoscalar meson, $P$,
\begin{equation}
    \Gamma^{(3)\,P}_{J_\mu}(t,t_J,\mathbf{p},\mathbf{k})=\int d^3\mathbf{x}\,
    e^{-i\mathbf{q}\cdotp\mathbf{x}}\,
    \langle{\phi_{P}(t,\mathbf{p})
    J_{\mu}(t_J,\mathbf{x})\phi^{\dagger}_{P}(0,\mathbf{k})}\,\rangle
\end{equation}
has the following asymptotic behavior for
$0\ll t_J\ll t$:
\begin{equation}
\begin{split}
    \Gamma^{(3)\,P}_{J_\mu}(t,t_J,\mathbf{p},\mathbf{k})=&\,L^3
    \frac{Z_P(\mathbf{p})Z_P(\mathbf{k})^{\dagger}\mathcal{M}_{J_\mu}^{P}(\mathbf{p},\mathbf{k})}
    {4E_{P}(\mathbf{p})E_{P}(\mathbf{k})}\\
     &\times e^{-(t-t_J)E_{P}(\mathbf{p})}e^{-t_JE_{P}(\mathbf{k})}\,
    \label{eq:GJasymp}
\end{split}
\end{equation}
where $\mathcal{M}_{J_\mu}^{P}
(\mathbf{p},\mathbf{k})=\bra{P(\mathbf{p})}
J_{\mu}(0)\ket{P(\mathbf{k})}$. This correlator is calculated for both the pion and the kaon.

\section{\label{sec:ama} Variance reduction techniques}

To compute the costly loop diagrams we use a variation of the all-mode-averaging (AMA) technique. On each configuration, for a given operator $\mathcal{O}$, we have an estimator $\mathcal{O}^{\textrm{e}}_{t_j}$ at ``exact" solver precision ($10^{-8}$, $10^{-10}$, $10^{-12}$, and $10^{-14}$ for the light, $c_{1}$, $c_{2}$, and $c_{3}$ quarks, respectively) using $T$ source times $t_j$ and a sparse noise $n_0$. We furthermore have $N$ estimators $\mathcal{O}^{\textrm{ie}}_{t_j, n_i}$ on each source time $t_j$ at ``inexact" solver precision ($10^{-4}$ for all quarks), computed for $N-1$ sparse noise sources $n_i$ in addition to the noise source $n_0$. The AMA estimator we construct from those estimators is
\begin{align}
    \mathcal{O}^{\textrm{zM}}_{t_j} = \left( \mathcal{O}^{\textrm{e}}_{t_j} - \mathcal{O}^{\textrm{ie}}_{t_j, n_0} \right) + \frac{1}{N-1} \sum_{i=1}^{N} \mathcal{O}^{\textrm{ie}}_{t_j, n_i}
    \, ,
\end{align}
where the superscript "zM" highlights that so far, the zM\"obius action has been used.  In a second AMA step, we compute a single estimator $\mathcal{O}^{\textrm{M}}$ for the sparse noise source $n_0$ and source time $t_0$ at ``exact" precision to get our final estimator
\begin{align}
    \mathcal{O} = \left(\mathcal{O}^{\textrm{M}} - \mathcal{O}^{\textrm{zM}}_{t_0}\right) + \frac{1}{T-1} \sum_{j =1}^{T} \mathcal{O}^{\textrm{zM}}_{t_j}
    \, .
\end{align}
The resulting expectation value $\langle \mathcal{O} \rangle = \langle \mathcal{O}^M \rangle$, but at a much reduced variance. In practice, we used $N=10$ and $T=6$, where the 6 source times have been chosen to evenly interlace the time extent of our lattice (16 timeslices apart from each other).

\section{\label{sec:fit_pars}Fit Parameters}%
Results of the decay amplitude are derived from global fits over all correlation functions involved in a specific fit strategy. A summary of the fit parameters for the 2pt and 3pt functions used, consistent across all fit strategies that they enter, is given in Table~\ref{tab:fit_pars}. The range of $T_a$ and $T_b$ used in each case is given in Table~\ref{tab:A0_results-supp}. In Fig.~\ref{fig:corrHeat} we show the correlation matrix of the 2pt and 3pt functions, as well as slices of the integrated 4pt function, which highlights the high degree of correlation between elements of the integrated 4pt function. This correlation structure in the data makes the use of uncorrelated fits for the integrated 4pt function necessary.

\begin{figure*}[t]
    \begin{centering}
        \includegraphics[width=0.75\textwidth]{./figures/corrHeat}
    \par\end{centering}
\protect\caption{\label{fig:corrHeat}The correlation matrix for the simultaneous fit used to extract $A_{0}$. The correlators in this fit are: the 2pt pion correlator with zero momentum and a point- $(\pi_{0}^{P})$ wall-sink $(\pi_{0}^{W})$, the equivalent correlators with one unit of momentum $(\pi_{1}^{P},~\pi_{1}^{W})$, the same again for the kaon $(K_{0}^{P},~K_{0}^{W},~K_{1}^{P},~K_{1}^{W})$, the vector current inserted on the pion $(3^{pt}_{\pi})$ and kaon $(3^{pt}_{K})$, the 3pt weak Hamiltonian correlator with zero $(H_{W}^{0})$ and one unit of momentum $(H_{W}^{1})$, and the integrated 4pt correlator $(I_{0}^{(4)})$. This shows the correlation matrix for a fully correlated fit. %However, 
Due to the highly correlated nature of the matrix, off-diagonal elements for the integrated 4pt function were set to zero to make the unintegrated 4pt function ``uncorrelated" to the other fit variables.}
\end{figure*}

\begin{table*}[t]
\caption{\label{tab:fit_pars}%
Fit parameters for the various 2pt and 3pt correlators and methods used to extract the $K^{+}\to\pi^{+}\ell^{+}\ell^{-}$ decay amplitude. With the exception of 3pt $c_{s}$ each of these were correlated to each other for the relevant simultaneous fits with the integrated 4pt function. The $c_{s}$ parameter was fitted separately and used as an input to the $c_s$ shift and $c_s\times\bar{s}d$ analyses. The 3pt $H_{W}$ and $c_{s}$ fit parameters are the same for the three unphysical charm-quark masses. ``Thinning" is the stride between data points entering the fit within the fit range.
}
\begin{ruledtabular}
\begin{tabular}{lcccccc}
Correlator&
Momentum&
Sink&
\textrm{$t_{src}$}&
\textrm{$t_{i}$}&
\textrm{$t_{f}$}&
Thinning\\
\colrule
\hline
 2pt pion & $\frac{2\pi}{L}(0,0,0)$ & Point & 32 & 7 & 18  & 2 \\
 2pt pion & $\frac{2\pi}{L}(0,0,0)$ & Wall & 32 & 13 & 20  & 2 \\
 2pt pion & $\frac{2\pi}{L}(1,0,0)$ & Point & 32 & 6 & 25  & 2 \\
 2pt pion & $\frac{2\pi}{L}(1,0,0)$ & Wall & 32 & 9 & 22  & 2 \\
 2pt kaon & $\frac{2\pi}{L}(0,0,0)$ & Point & 0 & 10 & 23  & 2 \\
 2pt kaon & $\frac{2\pi}{L}(0,0,0)$ & Wall & 0 & 9 & 20  & 2 \\
 2pt kaon & $\frac{2\pi}{L}(1,0,0)$ & Point & 0 & 11 & 26  & 2 \\
 2pt kaon & $\frac{2\pi}{L}(1,0,0)$ & Wall & 0 & 10 & 25  & 2 \\
 3pt pion & - & Wall & 0 & 1 & 10  & 2 \\
 3pt kaon & - & Wall & 0 & 20 & 35  & 2 \\
 3pt $c_{s}$ & $\frac{2\pi}{L}(0,0,0)$ & Wall & 0 & 9 & 24  & 1 \\
 3pt $H_{W}$ & $\frac{2\pi}{L}(0,0,0)$ & Wall & 0 & 17 & 24  & 2 \\
 3pt $H_{W}$ & $\frac{2\pi}{L}(1,0,0)$ & Wall & 0 & 13 & 17  & 1 \\
\hline
\end{tabular}
\end{ruledtabular}
\end{table*}

\begin{table*}[t]
\caption{\label{tab:A0_results-supp}%
Fit parameters for the various methods of extracting $A_{0}$. No thinning was performed on the integrated 4pt function data---meaning that all data points within the fit range entered the fit---which were uncorrelated when fitted simultaneously with the relevant 2pt and 3pt correlators.
}
\begin{ruledtabular}
\begin{tabular}{lcccc}
Analysis&
\textrm{$T_{a}$ min}&
\textrm{$T_{a}$ max}&
\textrm{$T_{b}$ min}&
\textrm{$T_{b}$ max}\\
\colrule
\hline
 Direct fit & 2  & 10  & 4 & 11 \\
\hline
 2pt/3pt recon & 1 & 10 & 7 & 15 \\
\hline
 0 mom transfer & 1 & 12 & 3 & 8 \\
\hline
 $SU(3)$ symm lim & 1  & 10  & 6 & 13 \\
\hline
 $c_s$ shift & 1 & 8 & 5 & 12 \\
\end{tabular}
\end{ruledtabular}
\end{table*}

\clearpage 


%\bibliography{rkSupMat}% Produces the bibliography via BibTeX.


